RT-Sketch: Goal-Conditioned Imitation Learning from Hand-Drawn Sketches

Natural language and images are commonly used as goal representations in goal-conditioned imitation learning (IL). However, natural language can be ambiguous and images can be over-specified. In this work, we propose hand-drawn sketches as a modality for goal specification in visual imitation learning. Sketches are easy for users to provide on the fly like language, but similar to images they can also help a downstream policy to be spatially-aware and even go beyond images to disambiguate task-relevant from task-irrelevant objects. We present RT-Sketch, a goal-conditioned policy for manipulation that takes a hand-drawn sketch of the desired scene as input, and outputs actions. We train RT-Sketch on a dataset of paired trajectories and corresponding synthetically generated goal sketches. We evaluate this approach on six manipulation skills involving tabletop object rearrangements on an articulated countertop. Experimentally we find that RT-Sketch is able to perform on a similar level to image or language-conditioned agents in straightforward settings, while achieving greater robustness when language goals are ambiguous or visual distractors are present. Additionally, we show that RT-Sketch has the capacity to interpret and act upon sketches with varied levels of specificity, ranging from minimal line drawings to detailed, colored drawings. For supplementary material and videos, please refer to our website: http://rt-sketch.github.io.

==> tex/3-problem.tex <==
% \subsection{Preliminaries}

\paragraph{Goal-Conditioned Imitation Learning} Our goal is to learn a manipulation policy conditioned on a goal \emph{sketch} of the desired scene state and a history of interactions. Formally, we denote such a policy by $\pi_{\mathrm{sketch}}(a_t | g, \{o_j\}^t_{j=1})$, where $a_t$ denotes an action at timestep $t$, $g \in \mathbb{R}^{W \times H \times 3}$ is a given goal sketch with width $W$ and height $H$, and $o_t \in \mathbb{R}^{W \times H \times 3}$ is an observation at time $t$. At inference time, the policy takes  given goal sketch along with a history of RGB image observations and infers an action to execute. In practice, we condition  $\pi_{\mathrm{sketch}}$ on a history of $H$ previous observations rather than all observations from $t=1$. To train such a policy, we consider learning from a dataset $\mathcal{D}_{\pi_{\mathrm{sketch}}} = \{(g^{n}, \{(o_t^{n}, a_t^{n})\}^{T^{(n)}}_{t=1}\}^{N}_{n=1}$ of $N$ successful demonstrations, where $T^{(n)}$ refers to the length of the n$^{th}$ trajectory in timesteps. Each episode of the dataset consists of a given goal sketch and a corresponding demonstration trajectory, with image observations recorded at each timestep. We leverage behavioral cloning~\citep{torabi2018behavioral}, which aims to reduce the negative log-likelihood of unfavorable actions $a_t$ under the distribution of goals and images induced by the training data.

\paragraph{RT-1} RT-1 is a prior language-to-action imitation learning agent trained on a large-scale dataset ($80$K trajectories) of VR-teleoperated demonstrations that include skills like moving objects near one another, placing cans and bottles upright or sideways, opening and closing cabinets, and performing pick and place on countertops and drawers~\citep{brohan2022rt}. In this work, we repurpose the RT-1 dataset but adapt the policy architecture to accommodate sketches, detailed below in \cref{sec:method}.


% In our setting, we consider goals provided as sketches rather than language instructions. To accommodate this change at the input, we omit the FiLM language tokenization altogether. Instead, we concatenate a given goal sketch with the history of images as input to EfficientNet, and extract tokens from this output, leaving the rest of the policy architecture unchanged. 



==> tex/5-experiments_figure_main.tex <==
\begin{figure}[ht]
    \newcommand{\headercellwidth}{.05cm}
    \newcommand{\imagecellwidth}{2.25cm}
    \newcommand{\imagesize}{0.15}
    %\setlength{\tabcolsep}{1pt}
    \centering
        \begin{tabular}{
        >{\centering\arraybackslash}m{\headercellwidth}
        >{\centering\arraybackslash}m{\imagecellwidth}
        >{\centering\arraybackslash}m{\imagecellwidth}
        >{\centering\arraybackslash}m{\imagecellwidth}
        >{\centering\arraybackslash}m{\imagecellwidth}
        >{\centering\arraybackslash}m{\imagecellwidth}}
            %==== row ====%
            (i) &
            \includegraphics[scale=\imagesize]{figures_tables/images/dummy/dummy_reference_initial_image.png} &
             \includegraphics[scale=\imagesize]{figures_tables/images/dummy/dummy_reference_goal_image.png} &
            \includegraphics[scale=\imagesize]{figures_tables/images/dummy/dummy_actual_initial_image.png} &
            \includegraphics[scale=\imagesize]{figures_tables/images/dummy/dummy_goal_sketch_image.png} &
            \includegraphics[scale=\imagesize]{figures_tables/images/dummy/dummy_achieved_goal_image.png} \\
            %==== row ====%
            (ii) &
            \includegraphics[scale=\imagesize]{figures_tables/images/dummy/dummy_reference_initial_image.png} &
             \includegraphics[scale=\imagesize]{figures_tables/images/dummy/dummy_reference_goal_image.png} &
            \includegraphics[scale=\imagesize]{figures_tables/images/dummy/dummy_actual_initial_image.png} &
            \includegraphics[scale=\imagesize]{figures_tables/images/dummy/dummy_goal_sketch_image.png} &
            \includegraphics[scale=\imagesize]{figures_tables/images/dummy/dummy_achieved_goal_image.png} \\
            %==== row ====%
           ~ & Reference initial image & Reference goal image & Actual initial image & Sketch goal image & Achieved goal image \\
            %==== row ====%
           ~ & (a) & (b) & (c) & (d) & (e)
        \end{tabular}
    \caption{Main figure of qualitative results.}
    \label{fig:main}
\end{figure}

==> tex/5-experiments_table_main.tex <==
\begin{table}[ht]
    \newcommand{\hypcellwidth}{0.3cm}
    \newcommand{\methodcellwidth}{2.7cm}
    \newcommand{\cellwidth}{1cm}
    \setlength{\tabcolsep}{3pt}
%    \renewcommand{\arraystretch}{1.}
    \centering
    \scriptsize
    \begin{tabular}{
        >{\centering\arraybackslash}m{\hypcellwidth}
        m{\methodcellwidth}
        >{\centering\arraybackslash}m{\cellwidth}
        >{\centering\arraybackslash}m{\cellwidth}
        >{\centering\arraybackslash}m{\cellwidth}
        >{\centering\arraybackslash}m{\cellwidth}
        >{\centering\arraybackslash}m{\cellwidth}
        >{\centering\arraybackslash}m{\cellwidth}
        >{\centering\arraybackslash}m{\cellwidth}}
        \hline
        %==== row ====%
        & &  \multicolumn{7}{c}{{\bf Skill}} \\
        & {\bf Method}  & \movenear & \knock & \upright & \opendrawer & \closedrawer & \drawerpick & \drawerplace \\
        \hline
        %==== row ====%
        \multirow{4}{\cellwidth}{{\em H1}} & \rtsketch  & $0/0$ & $0/0$ & $0/0$ & $0/0$ & $0/0$ & $0/0$ & $0/0$ \\
        & \rtone~\citep{brohan2022rt}                   & & & & & & & \\
        & \rtsketchgoalimage                            & & & & & & & \\
        & \rtonegoalimage                               & & & & & & & \\
        \hline
        %==== row ====%
        \multirow{4}{\cellwidth}{{\em H2}} & \rtsketch  & $0/0$ & $0/0$ & $0/0$ & $0/0$ & $0/0$ & $0/0$ & $0/0$ \\
        & \rtone~\citep{brohan2022rt}                   & & & & & & & \\
        & \rtsketchgoalimage                            & & & & & & & \\
        & \rtonegoalimage                               & & & & & & & \\
        \hline
        %==== row ====%
        \multirow{4}{\cellwidth}{{\em H3}} & \rtsketch  & $0/0$ & $0/0$ & $0/0$ & $0/0$ & $0/0$ & $0/0$ & $0/0$ \\
        & \rtone~\citep{brohan2022rt}                   & & & & & & & \\
        & \rtsketchgoalimage                            & & & & & & & \\
        & \rtonegoalimage                               & & & & & & & \\
        \hline
        %==== row ====%
        \multirow{4}{\cellwidth}{{\em H4}} & \rtsketch  & $0/0$ & $0/0$ & $0/0$ & $0/0$ & $0/0$ & $0/0$ & $0/0$ \\
        & \rtone~\citep{brohan2022rt}                   & & & & & & & \\
        & \rtsketchgoalimage                            & & & & & & & \\
        & \rtonegoalimage                               & & & & & & & \\
        \hline
    \end{tabular}
    \caption{Main table of quantitative results.}
    \label{tab:main}
\end{table}

